Towards Global Optimality for Practical Average Reward Reinforcement Learning without Mixing Time Oracles

In the context of average-reward reinforcement learning, the requirement for oracle knowledge of the mixing time, a measure of the duration a Markov chain under a fixed policy needs to achieve its stationary distribution, poses a significant challenge for the global convergence of policy gradient methods. This requirement is particularly problematic due to the difficulty and expense of estimating mixing time in environments with large state spaces, leading to the necessity of impractically long trajectories for effective gradient estimation in practical applications. To address this limitation, we consider the Multi-level Actor-Critic (MAC) framework, which incorporates a Multi-level Monte-Carlo (MLMC) gradient estimator. With our approach, we effectively alleviate the dependency on mixing time knowledge, a first for average-reward MDPs global convergence. Furthermore, our approach exhibits the tightest available dependence of $\mathcal{O}\left( \sqrt{\tau_{mix}} \right)$known from prior work. With a 2D grid world goal-reaching navigation experiment, we demonstrate that MAC outperforms the existing state-of-the-art policy gradient-based method for average reward settings.

==> arxiv_sections/preliminaries.tex <==
\subsection{Preliminaries} \label{section:prelim}
In this section, we provide assumptions and lemmas that will support our global convergence analysis in the next section.
\begin{assumption}
    \label{assumption:erogidcity}
    For all $\theta$, the parameterized MDP $\mathcal{M_{\theta}}$ induces an ergodic Markov Chain.
\end{assumption}

Assumption \ref{assumption:erogidcity} is typical in many works such as \cite{suttle2023beyond, pesquerel2022imed,gong2020duality, bai2023regret}. As previously mentions, it ensures all states are reachable, and also importantly, guarantees a unique stationary distribution $d^{\pi_{\theta}}$ of any induced Markov Chain. 

% \textcolor{red}{All this text from here to right before assumption 4.3 is copied from icml mac paper. wasn't sure the best way to reduce this. i just need to introduce the critic error approximation but not sure how much of this can be taken out}
% The algorithmic setting considered in this paper is that of actor-critic with linear function approximation, where the critic updates correspond to using TD(0) \cite{sutton2018reinforcement} to estimate the state value function. Specifically, we assume that, for a given critic parameter $\omega \in \mathbb{R}^k$ and state $s$, our critic approximator is of the form $V_{\omega}(s) = \phi(s)^T \omega$ [cf. \eqref{value_function_problem}, where $\phi : \mathcal{S} \rightarrow \mathbb{R}^k$ is a given feature mapping that we assume satisfies $\sup_s \norm{ \phi(s) } \leq 1$.

% As discussed in Ch. 9 of \cite{sutton2018reinforcement}, for a fixed policy parameter $\theta$, TD(0) with linear function approximation will converge to the minimum of the mean squared projected Bellman error (MSPBE), which satisfies
%
% \begin{equation}\label{critic_colution}
%     A_{\theta} \omega = b_{\theta},
% \end{equation}
%     %
% \begin{equation}
%     A_{\theta} = \mathbf{E}_{s \sim \mu_{\theta}, a \sim \pi_{\theta}, s' \sim p(\cdot | s, a)} \left[ \phi(s) (\phi(s) - \phi(s'))^T \right], \nonumber
% \end{equation}
% %
% \begin{equation}
%     b_{\theta} = \mathbf{E}_{s \sim \mu_{\theta}, a \sim \pi_{\theta}} \left[ ( r(s, a) - J(\theta) ) \phi(s) \right]. \nonumber
% \end{equation}
%
% In what follows, we will use $\omega^*(\theta)$ to denote the fixed point satisfying Eq. \eqref{critic_colution} for a given $\theta$. We will also use $\omega^*_t = \omega^*(\theta_t)$ to denote the fixed point associated with policy parameter vector $\theta_t$ at time $t$.

%

%
Because we parameterize the critic as a linear function approximator, for a fixed policy parameter $\theta$, the temporal difference will converge to the minimum of the mean squared projected Bellman error (MSPBE) as discussed in \cite{sutton2018reinforcement}.  
\begin{definition}\label{assum:mspbe}
Denoting $\omega^*(\theta)$ as the fixed point for a given $\theta$, and for a given feature mapping $\phi$ for the critic, we define the worst-case approximation error to be
\begin{align}
    \mathcal{E}^{critic}_{app} = \sup_{\theta} \sqrt{ \mathbf{E}_{s \sim \mu_{\theta}} \left[ \phi(s)^T \omega^*(\theta) - V^{\pi_{\theta}}(s) \right]^2},
\end{align}
\end{definition}

%
which we assume to be finite. With a well-designed feature map, $\mathcal{E}^{critic}_{app}$ will be small or even 0. We will later see that by assuming $\mathcal{E}^{critic}_{app} = 0$ we recover the $\wo{T^{-\frac{1}{4}}}$ dependence as in \cite{bai2023regret}. 

% Intuitively, $\mathcal{E}^{critic}_{app}$ quantifies the quality of the feature mapping: when the features are well-designed, $\mathcal{E}^{critic}_{app}$ will be small or even 0, while poorly designed features will tend to have higher worst-case error.

% Analyses of TD learning typically assume positive definiteness of the matrices $A_{\theta}$ to ensure the solvability of the MSPBE minimization problem and uniqueness of its solutions \cite{bhandari2018, zou2019finite, qiu2021finite}, which we subsequently impose via Assumption \ref{assum:critic_positive_definite}.
% %
% \begin{assumption} \label{assum:critic_positive_definite}
%     There exist $\lambda > 0$ such that, for all $\theta$, the matrix $A_{\theta}$ is positive definite, its eigenvalues are all bounded and have norm greater than or equal to $\lambda$.
% \end{assumption}

% As indicated in our description of the algorithm in the previous section, we execute a projection onto a norm-ball with radius $R_{\omega} > 0$, denoted by set $\Omega$, in our critic update step [cf. \eqref{Critic_update_MAC}]. As mentioned in \cite{wu2020finite}, given Assumption \ref{assum:critic_positive_definite}, we can simply take $R_{\omega} = 2 R / \lambda$, since $\norm{b_{\theta}} \leq 2R$ by the boundedness of rewards, and $\norm{A_{\theta}^{-1}} \leq 1 / \lambda$.


\begin{assumption} \label{assum:policy_conditions}
    Let $\{ \pi_{\theta} \}_{\theta \in \mathbb{R}^d}$ denote our parameterized policy class. There exist $B, R, L > 0$ such that
    %
    \begin{enumerate}
        \setlength\itemsep{0em}
        \item $\norm{ \nabla \log \pi_{\theta}(a | s) } \leq B$, for all $\theta \in \mathbb{R}^d$,
        %
        \item $\norm{ \nabla \log \pi_{\theta}(a | s) - \nabla \log \pi_{\theta'}(a | s) } \leq R \norm{ \theta - \theta' }$, for all $\theta, \theta' \in \mathbb{R}^d$,
        %
        \item $| \pi_{\theta}(a | s) - \pi_{\theta'}(a | s) | \leq L \norm{\theta - \theta'}$, for all $\theta, \theta' \in \mathbb{R}^d$.
    \end{enumerate}
\end{assumption}

Assumption \ref{assum:policy_conditions} establishes regularization conditions for the policy gradient ascent and has been utilized in prior work such as \cite{suttle2023beyond, papini2018stochastic, kumar2019sample, zhang2020global, xu2020improved, bai2023regret}. This assumption will be vital for presenting our modified general framework for non-constant stepsize in Lemma \ref{lem_framework} as $B, R, L$ will appear in our bound for the difference between optimal reward and the average cumulative reward.

\begin{assumption}
    \label{assump_transfer_error}
    Define the transferred policy function approximation error
    \begin{align}
        \label{eq:transfer_error}
        \begin{split}
            L_{d_\rho^{\pi^*},\pi^*}(h^*_\theta,\theta &) =\mathbf{E}_{s\sim d_\rho^{\pi^*}}\mathbf{E}_{a\sim\pi^*(\cdot\vert s)}\bigg[\\
            &\bigg(\nabla_\theta\log\pi_{\theta}(a\vert s)\cdot h^*_{\theta}-A^{\pi_\theta}(s,a)\bigg)^2\bigg],
	\end{split}
    \end{align}
    where $\pi^*$ is the optimal policy and $h^*_{\theta}$ is given as
    \begin{align}
        \label{eq:NPG_direction}
	\begin{split}
            h^*_{\theta}=\arg&\min_{h\in\mathbb{R}^{\mathrm{d}}}~\mathbf{E}_{s\sim d_\rho^{\pi_{\theta}}}\mathbf{E}_{a\sim\pi_{\theta}(\cdot\vert s)}\bigg[\\
            &\bigg(\nabla_\theta\log\pi_{\theta}(a\vert s)\cdot h-A^{\pi_{\theta}}(s,a)\bigg)^2\bigg].
	\end{split}
    \end{align}
    We assume that the error satisfies $L_{d_{\rho}^{\pi^*},\pi^*}(h^*_{\theta},\theta)\leq \mathcal{E}^{actor}_{app}$ for any $\theta\in\Theta$ where $\mathcal{E}^{actor}_{app}$ is a positive constant.
\end{assumption}

Assumption \ref{assump_transfer_error} bounds the error that arises from the policy class parameterization. For neural networks, $\mathcal{E}^{actor}_{app}$ has shown to be small \citep{wang2019neural}, while for softmax policies, $\mathcal{E}^{actor}_{app} = 0$ \citep{agarwal2021theory}. This approximation assumption has also been used in \cite{bai2023regret}, and is important to generalizing the policy parameterization in the convergence analysis  we will later see in Section \ref{section:global_convergence} as $\mathcal{E}^{actor}_{app}$ will appear as its own independent term in the final bound.
% \textcolor{cyan}{can our experiments show any ablation study with respect to these assumptions? especially Assumption \ref{assum:mspbe} - \ref{assump_transfer_error} look very technical, so we should visualize how performance changes as a function of the chosen feature map for the critic, as well as policy parameterization, so we have some rough characterization in practice.} 
% \textcolor{red}{I remember we discussed if this approximaiton assumption holds for MLMC, and it should. however, i'm iffy if it holds for actor-critic. i think it should because the temporal difference estimation of the critic is supposed to be an estimaiton of the advantage. }

For our later analysis, we also define 
\small
    \begin{align}
      %  \begin{split}
            F(\theta)=
            \mathbf{E}_{s\sim d^{\pi_{\theta}}}\mathbf{E}_{a\sim\pi_{\theta}(\cdot\vert s)}\left[\nabla_{\theta}\log\pi_{\theta}(a|s)(\nabla_{\theta}\log\pi_{\theta}(a|s))^T \right],\nonumber
    \end{align}
\normalsize
as the Fisher information matrix. We can now also express $h^*_\theta$ defined in \eqref{eq:NPG_direction} as,
    \begin{align*}
        h^*_{\theta} = F(\theta)^{\dagger} \mathbf{E}_{s\sim d^{\pi_{\theta}}}\mathbf{E}_{a\sim\pi_{\theta}(\cdot\vert s)}\left[\nabla_{\theta}\log\pi_{\theta}(a|s)A^{\pi_{\theta}}(s, a)\right],
    \end{align*}
where $\dagger$ denotes the Moore-Penrose pseudoinverse operation.
% \begin{remark}
%     $h^*_\theta$ defined in \eqref{eq:NPG_direction} can be also be expressed in terms of the Fisher information matrix,
%     \begin{align*}
%         h^*_{\theta} = F(\theta)^{\dagger} \mathbf{E}_{s\sim d^{\pi_{\theta}}}\mathbf{E}_{a\sim\pi_{\theta}(\cdot\vert s)}\left[\nabla_{\theta}\log\pi_{\theta}(a|s)A^{\pi_{\theta}}(s, a)\right]
%     \end{align*}
%     where $\dagger$ symbolizes the Moore-Penrose pseudoinverse operation and $F(\theta)$ is the Fisher information matrix as defined below.
%     \begin{align}
%         \begin{split}
%             F(\theta) = \mathbf{E}_{s\sim d^{\pi_{\theta}}}&\mathbf{E}_{a\sim\pi_{\theta}(\cdot\vert s)}\left[\right.\\
%             &\left.\nabla_{\theta}\log\pi_{\theta}(a|s)(\nabla_{\theta}\log\pi_{\theta}(a|s))^T\right]
%         \end{split}
%     \end{align}
% \end{remark}

\begin{assumption}
    \label{assump_4}
    Setting $I_{F}$ as the identity matrix of same dimensionality as $F(\theta)$, let there exists some positive constant $\mu_F$ such that $F(\theta)-\mu_F I_{F}$ is positive semidefinite.
\end{assumption}
Assumption \ref{assump_4} is a common assumption for global convergence of policy gradient algorithms \cite{liu2020improved, bai2023regret}. This assumption will be useful later in our analysis by translating the general framework proposed in Lemma \ref{lem_framework} into terms of $\left[ \bignorm{ \nabla J(\theta_t) }^2 \right]$, the local convergence rate of MAC. We then can use the convergence rate bound established by \cite{suttle2023beyond}, which we state in Lemma \ref{lemma:convergence_rate}.

% which MAC has an bound for established by \cite{suttle2023beyond}. We provide that bound in Lemma \ref{lemma:convergence_rate}. 
% \textcolor{cyan}{how are these lemmas intertwined, what role do they play in the overall analysis, and which steps of their proof are interesting/innovative? remind me before/after each one is presented}

% \begin{lemma} \label{lemma:a6ss}
% %
% Assume $\norm{ \nabla J(\theta) }, \norm{ \nabla J_t^{i, \eta, V} } \leq G_H$, for all $\theta, s_t^i, a_t^i$. Fix $T_{max} \in \mathbb{N}$ and let $K = \tau_{max}^{\theta_t} \lceil 2 \log T_{max} \rceil$. Define $h_t^N = \frac{1}{N} \sum_{i=1}^N \nabla J_t^i$, for $N \in \left[ T_{max} \right]$. Then, for all $N \in \left[ T_{max} \right]$ and $\theta_t$ measurable w.r.t. $\mathcal{F}_{t-1}$,
% %
% \small
% \begin{align}
%     % \mathbb E \left[ \norm{h_t^N - \nabla J(\theta_t)} \right] &\leq O \left( G_H \sqrt{\log KN} \sqrt{\frac{K}{N}} \right) + \mathcal{E}_1(t) + 2B \mathcal{E}^{critic}_{app}, \\
%     %
%     \mathbb E \left[ \norm{ h_t^N - \nabla J(\theta_t) }^2 \right] &\leq O \left( G_H^2 \log(KN)\frac{K}{N} \right)  \\ &+\mathcal{E}_2(t) + 16 B^2 \mathcal{E}^{critic}_{app},
% \end{align}
% %
% \normalsize
% where
% %
% \small
% \begin{align}
%     % \mathcal{E}_1(t) &= B \mathbb{E} \left[ \norm{ \eta_t - \eta_t^* } \right] + BC \mathbb{E} \left[ \norm{\omega_t - \omega_t^*} \right], \label{eqn:a6ss_1} \\
%     %
%     \mathcal{E}_2(t) &= 4B^2 \mathbb{E} \left[ \norm{ \eta_t - \eta_t^* }^2 \right] + 4B^2C^2 \mathbb{E} \left[ \norm{\omega_t - \omega_t^*}^2 \right]. \label{eqn:a6ss_2}
% \end{align}
% %
% \normalsize
% \end{lemma}

\begin{lemma} \label{lemma:31ss}
%
Let $j_{max} = \floor{\log T_{max}}$. Fix $\theta_t$ measurable w.r.t. $\mathcal{F}_{t-1}$. Assume $T_{max} \geq \tau_{mix}^{\theta_t}$, $\norm{\nabla J(\theta)} \leq G_H$, for all $\theta$, and $\norm{ h_t^N } \leq G_H$, for all $N \in \left[ T_{max} \right]$. Then
%
\small
\begin{align}
    \mathbf{E}_{t-1} \left[ h_t^{MLMC} \right] &= \mathbf{E}_{t-1} \left[ h_t^{j_{max}} \right], \label{eqn:31ss_mean} \\  
    \mathbf{E} \left[ \norm{ h_t^{MLMC} }^2 \right] &\leq \wo{ G_H^2 \tau_{mix}^{\theta_t} \log T_{max} } \nonumber\\&+ 8 \log(T_{max}) T_{max} \left( \mathcal{E}(t) + 16B^2 (\mathcal{E}^{critic}_{app})^2 \right)  \label{eqn:31ss_2nd_moment} \\ 
    \mathbf{E} \norm{\nabla J(\theta_t)-h&_t^{j_{max}}}^2  \leq \wo{ G_H^2 \tau_{mix}^{\theta_t} \frac{\log T_{max}}{T_{max}} } \nonumber\\& +  \mathcal{E}_2(t) +  16B^2 (\mathcal{E}^{critic}_{app})^2. \label{eqn:est_err_variance}
     % \E \left[ \norm{\nabla J(\theta_t) &- h_t^{j_{max}}}^2 \right] \leq \wo{ G_H^2 \tau_{mix}^{\theta_t} \frac{\log T_{max}}{T_{max}} } \nonumber \\+  \mathcal{E}_2(t) +  16B^2 (\mathcal{E}^{critic}_{app})^2.
\end{align}
%
\normalsize
\end{lemma}

Lemma \ref{lemma:31ss} provides a bound for the variance of the MLMC gradient estimator and will be integral to our analysis.

% \textcolor{red}{Due to definition of MLMC estimator where we $2^{J_t}(h^{J_t} - h^{J_t - 1})$, the $2^{J_t}$ is what creates the extra $T_{\max}$ in the second term of the expected variance bound. This causes trouble when trying to recover the $\bo{T^{-\frac{1}{4}}}$ bound in vaneet's paper}

\begin{lemma} \label{thm:critic_analysis_main_body}
Let $\beta_t = \gamma_t = (1 + t)^{-\nu}, \alpha = \alpha_t' / \sqrt{\sum_{k=1}^t \norm{h^{MLMC}_t}^2}$, and $\alpha_t' = (1 + t)^{-\sigma}$, where $0 < \nu < \sigma < 1$. Then
%
\small
\begin{align}
    \frac{1}{T} &\sum_{t=1}^T  \mathcal{E}(t) \leq \bo{T^{\nu - 1}} + \bo{T^{-2(\sigma - \nu)}} \nonumber\\
    %
    &+ \wo{  \tau_{mix} \log T_{\max}} \bo{T^{-\nu}} \nonumber\\&+ \wo{  \tau_{mix} \frac{\log T_{\max}}{T_{\max}} }. 
    %
    % &+ \wo{ \sqrt{ \max_{t \in [T]} \tau_{mix}^{\theta_t} \frac{\log T_{\max}}{T_{\max}} } } \\
    %
    % &\quad+ \wo{  \tau_{mix} \frac{\log T_{\max}}{T_{\max}} }. 
    \label{ineq:critic_1}
\end{align}
\normalsize

By setting $\nu = 0.5$ and $\sigma = 0.75$ leads to the following:
\small
\begin{align}
    \frac{1}{T} \sum_{t=1}^T  \mathcal{E}(t) \leq 
    % \bo{T^{-\frac{1}{2}}} + \bo{T^{-\frac{1}{2}}} \nonumber\\
    % %
    % &+ \wo{ \tau_{mix} \log T_{\max}} \bo{T^{-\frac{1}{2}}} \nonumber\\
    % %
    % % &+ \wo{ \sqrt{ \max_{t \in [T]} \tau_{mix}^{\theta_t} \frac{\log T_{\max}}{T_{\max}} } } \\
    % %
    % &\quad+ \wo{ \tau_{mix}\frac{\log T_{\max}}{T_{\max}} } = \nonumber\\ 
    &\wo{ \tau_{mix} \log T_{\max}} \bo{T^{-\frac{1}{2}}} \nonumber\\&+ \wo{ \tau_{mix}\frac{\log T_{\max}}{T_{\max}} }. \label{ineq:critic_2}
\end{align}
\normalsize

\end{lemma}

Lemma \ref{thm:critic_analysis_main_body} established by \cite{suttle2023beyond} states the convergence rate of the critic with an MLMC estimator. This result directly affects the overall MAC convergence rate from \cite{suttle2023beyond} stated below,

% \textcolor{red}{I think both $\bo{T^{-\frac{1}{2}}}$ can just disappear because of the $\wo{ \tau_{mix} \log T_{\max}} \bo{T^{-\frac{1}{2}}}$ term}

% In this section, we provide propositions and assumptions previously established that will be fundamental in our analysis. The folllowing proposition established by \cite{dorfman2022adapting} and adapted to actor-critic setting by \cite{suttle2023beyond} characterizes the mean and variance of the MLMC gradient estimator.

% \begin{proposition} \label{prop:31ss}
% %
% Let $j_{max} = \floor{\log T_{max}}$ in Algorithm \ref{algo:mlmc_pg}. Fix $\theta_t$ measurable w.r.t. $\mathcal{F}_{t-1}$. Assume $T_{max} \geq \tau_{mix}^{\theta_t}$, $\norm{\nabla J(\theta)} \leq G_H$, for all $\theta$, and $\norm{ h_t^N } \leq G_H$, for all $N \in \left[ T_{max} \right]$. Then
% %
% \begin{align}
%     \mathbb{E}_{t-1} \left[ h_t^{MLMC}\right] &= \mathbb{E}_{t-1} \left[ h_t^{j_{max}} \right], \label{eqn:31ss_mean} \\
%     %
%     \mathbb{E} \left[ \norm{ h_t^{MLMC} }^2 \right] &\leq \wo{ G_H^2 \tau_{mix}^{\theta_t} \log T_{max} }. \label{eqn:31ss_2nd_moment}
% \end{align}
% %
% \end{proposition}

% Using Proposition \ref{prop:31ss} leads to the next propositions that bounds the estimation error the MLMC gradient.

% \begin{proposition}\label{prop:grad_est_bound}
    
%     \begin{align}
%     \sum_{t=1}^T \mathbb E \left[ \norm{\nabla J(\theta_t) - h_t^{MLMC}}^2 \right] &\leq \\ &\wo{ T G_H^2 \tau_{mix}^{\theta_t} \frac{\log T_{max}}{T_{max}} }.
% \end{align}
% \end{proposition}

% We now state the convergence of the policy gradient norm in the average reward setting, adapting it from \cite{suttle2023beyond} for policy gradient algorithms in general, not just actor-critic. 

% \begin{proposition}
    
% \label{thm:actor_bd}
% Assume $J(\theta)$ is $L$-smooth, $\sup_{\theta} | J(\theta) | \leq M$, and $\norm{ \nabla J(\theta) }, \norm{ h_t^{MLMC} } \leq G_H$, for all $\theta, t$. Let $\alpha_t = \alpha_t' / \sqrt{ \sum_{t=1}^T \norm{h_t^{MLMC}}^2 }$, where $\{ \alpha_t' \}$ is an auxiliary stepsize sequence with $\alpha_t' \leq 1$, for all $t \geq 1$. Then
% %
% \small
% \begin{align}\label{actor_adagrad}
%     \frac{1}{T} \sum_{t=1}^T \mathbb{E} & \left[ \bignorm{ ||\nabla J(\theta_t)|| }^2 \right] \leq \bo{\frac{1}{\sqrt{T}} } + \wo{ \tau_{mix} \frac{\log T_{\max}}{T_{\max}}},
% \end{align}
% \normalsize
% \end{proposition}




\begin{lemma}(MAC Convergence Rate) \label{lemma:convergence_rate}
    Assume $J(\theta)$ is $L$-smooth, $\sup_{\theta} | J(\theta) | \leq M$, and $\norm{ \nabla J(\theta) }, \norm{ h_t^{MLMC} } \leq G_H$, for all $\theta, t$ and under assumptions of Lemma \ref{thm:critic_analysis_main_body}, we have
    %
    \begin{align}\label{final_mac_bound}
    \frac{1}{T} \sum_{t=1}^T \mathbb{E}
     \left[ \bignorm{ \nabla J(\theta_t) }^2 \right]\leq & \bo{ \mathcal{E}^{critic}_{app} }+\wo{ \frac{\tau_{mix} \log T_{\max}}{\sqrt{T}}} \nonumber
    \\
    &\hspace{-4mm} +\wo{ { \frac{\tau_{mix}\log T_{\max}}{T_{\max}}} } .
    \end{align}
    %
 
\end{lemma}
% {\bf \color{red}Explicitly mention which result or proof was wrong in Suttle paper, and what is fixed. Any key insight or novelty that came in the fix could also be mentioned. Cannot use "correct" without full explanation here - was Lemma 3 or 4 wrong?}

Both Lemmas \ref{thm:critic_analysis_main_body} and \ref{lemma:convergence_rate} rely on the convergence of the error in average reward tracking, provided in Lemma D.1 of \cite{suttle2023beyond}. However, we have noticed that there is a $\wo{ \sqrt{ \frac{\tau_{mix}\log T_{\max}}{T_{\max}}} }$ term in Lemma D.1 that should actually absorb the $\wo{ { \frac{\tau_{mix}\log T_{\max}}{T_{\max}}} }$ term in \ref{ineq:critic_2} and \ref{final_mac_bound}. We provide a correct version of the proof of Lemma D.1 in the Appendix where we were able to remove the square root. 


Finally, we will use the following result to manipulate the AdaGrad stepsizes in the final result of this section.
%
\begin{lemma}{Lemma 4.2, \citep{dorfman2022}.} \label{lemma:42}
For any non-negative real numbers $\{ a_i \}_{i \in [n]}$,
%
\begin{equation}
    \sum_{i=1}^n \frac{a_i}{ \sqrt{ \sum_{j=1}^i a_j } } \leq 2 \sqrt{ \sum_{i=1}^n a_i }.
\end{equation}
\end{lemma}

% \textcolor{red}{I think there is a typo from our icml paper. in the appendix from which i copied it from, there is a square root over the entire last term of this theorem. in the main body, there is none}



==> sections/conclusion.tex <==
\section{Conclusion and Further Work}
In this work, we provide policy gradient global convergence analysis for the infinite horizon average reward MDP without restrictive and impractical assumptions on mixing time. Using MAC, we show that actor-critic models, utilizing a MLMC gradient estimator, achieves a tighter dependence on mixing time for global convergence. We hope this work encourages further investigation into algorithms that do not assume oracle knowledge of mixing time. Future work can also further test the advantages of MAC in slow mixing environments for robotics, finance, healthcare, and other applications.

% \section*{Impact Statement}

% This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.


==> sections/experiments.tex <==
\subsection{Experimental Results}\label{section:experiments}

As a preliminary proof-of-concept experiment to show the advantage of MAC over PPGAE, Vanilla AC, and REINFORCE, we consider a $15$-by-$15$ sparse gridworld environment. The agent tries to from the top left to bottom right corner. The agent receives a reward of $+1$ if goal is reached and $+0$ else. The episode ends when the agent either reaches the goal or hits a limit of $200$ samples. We report a moving average success rate over $100$ trials with $95\%$ confidence intervals in Figure \ref{fig:experiments}. We can see that MAC has a higher success rate and can more consistently reach the goal than the baselines.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.85\columnwidth]{10x10.png}
    % \subfigure[]{\includegraphics[width=0.7\columnwidth]{tmax16_10x10_lr005.png}}
  \caption{Success Rate in a sparse $15$-by-$15$ grid over 300 training episodes with $200$ samples per episode. For MAC, $T_{max} = 4$ and for PPGAE, $H = 200$ and $N = 1$. Vanilla AC and REINFORCE both have $H = 200$. and $100$ trials for each algorithm. PPGAE, Vanilla AC, and REINFORCE consistently converge to significantly less optimal solutions than MAC.}
  \label{fig:experiments}
\end{figure}


% The intuition behind this sparse reward structure is to see which algorithm is better at exploring different actions when there is a higher incentive to stay than to move.




% In this section, we present preliminary experiments that compare MAC against Parameterized Policy Gradient with Advantage Estimation (PPGAE) from \cite{bai2023regret}.

% We consider multiple goal-conditioned navigation tasks in a sparse $n \times n$  gridworld domain environment where there are five action: stay, up, down, left, and right. The settings of the different tasks are explained as follows,

% \begin{itemize}
%     \item \textbf{Start Reset, Single Goal: }In every episode, the start is always the top left and the goal is the top right. The episode ends when the goal is reached or a maximum number of samples has been reached. The agent then resets to the top left at the beginning of each episode.

%     \item \textbf{Start Reset, Multi-Goal: }In every episode, the start is always top left but the goal changes to a random different location on the grid excluding the top left.

%     \item \textbf{Continuing Multi-Goal: }The agent in the first episode starts in the top left. The goal changes position every episode. The agent, however, starts the next episode where it ended up in the previous episode. 
    
% \end{itemize}

% For all the tasks we consider the same sparse reward structure: If the agent reaches the goal, it receives a positive reward of $+20$. For all other states it receives a reward of $0$.

==> sections/global_convergence.tex <==

\section{Global Convergence Analysis} 
In this section we provide theoretical guarantee of the global convergence of MAC from \cite{suttle2023beyond}. 
% \textcolor{red}{Bhrij comments: Maybe I'm misunderstanding but doesn't all the analysis including MAC's need to know mixing time. however, when the algorithm itself requires to know mixing time, that is a different story. } 
% \textcolor{cyan}{what are key steps in the prior analysis that require oracle knowledge of mixing time? how are these steps broken if we do not have this knowledge? how does our technical setting/algorithm alleviate these requirements? remind me again as incentive for understanding what our core theorem achieves. Also remind me what role this background information plays in paving the path towards achieving these results}

\label{section:global_convergence}
\input{sections/preliminaries}
\subsection{Global Convergence Guarantee}
To develop our convergence analysis, we present a modified version of the general framework proposed in \cite{bai2023regret} to accommodate non-constant stepsizes such as Adagrad. 
% Using Lemma \ref{lem_performance_diff}, we present a general framework for convergence analysis of the policy gradient algorithm in the averaged reward case as dictated below. This is inspired by the convergence analysis of \citep{liu2020improved} for the discounted reward MDPs. 

% \textcolor{red}{Below is a modified version of Lemma 5 from vaneet's paper where instead of constant stepsize $\alpha$, we have $\alpha_t$. This is to accommodate Adagrad. I'm not sure if we need to write a whole entire modified proof of Lemma 5}
\begin{lemma}
    \label{lem_framework} 
    Suppose a general gradient ascent algorithm updates the policy parameter in the following way.
    \begin{equation}
	\theta_{t+1}=\theta_t+\alpha_t h_t.
    \end{equation}
    When Assumptions \ref{assum:policy_conditions}, \ref{assump_transfer_error}, and \ref{assump_4} hold, we have the following inequality for any $T$.
    \begin{equation}
        \label{eq:general_bound}
	\begin{split}
            &J^{*}-\frac{1}{T}\sum_{t=1}^{T}J(\theta_t)\leq \sqrt{\mathcal{E}^{actor}_{app}}+\frac{B}{T}\sum_{t}^{T}\Vert(h_t-h^*_t)\Vert\\
            &+\frac{R}{2T}\sum_{t=1}^{T}\alpha_t\Vert h_t\Vert^2+\frac{1}{T}\sum_{t=1}^{T}\frac{1}{\alpha_t}\mathbf{E}_{s\sim d^{\pi^*}}\zeta_t,	
        \end{split}
    \end{equation}
    where $h^*_t:=h^*_{\theta_t}$ and $h^*_{\theta_t}$ is defined in \eqref{eq:NPG_direction}, $J^*=J(\theta^*)$, and $\pi^*=\pi_{\theta^*}$ where $\theta^*$ is the optimal parameter, and $\zeta_t = [KL(\pi^*(\cdot\vert s)\Vert\pi_{\theta_k}(\cdot\vert s))-KL(\pi^*(\cdot\vert s)\Vert\pi_{\theta_{k+1}}(\cdot\vert s))]$.
\end{lemma}

We provide a proof of the above lemma in Appendix \ref{lem_framework_proof}. The proof is similar to that of \cite{bai2023regret} with a notable difference that the non-constant stepsize does not allow us to simplify the telescoping summation in the last term without bounding $\alpha_t$ to some constant which we will do later in the analysis. 


% We can remove the $\sqrt{\mathcal{E}^{critic}_{app}}$ as it will be dominated by the ${\mathcal{E}^{critic}_{app}}$ term.\textcolor{red}{I think the second term of the RHS of \ref{convergence_rate_bound} can be absorbed into the first term of the RHS of \ref{variance_bound_sqrt_with_rt_T}}
% \textcolor{red}{I think we can ignore the $\sqrt{\frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\bigg[\Vert  h_t\Vert^2\bigg]}$ term as it will become negligible because of the $\frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\bigg[\Vert  h_t\Vert^2\bigg]$ term}
% \textcolor{red}{Also I haven't included $\alpha$ stepsize in this bound. Not sure if we need to worry about that or somehow include Adagrad bounds in this as well}
% \textcolor{cyan}{remind me why the theorem is establishing a result that is sharper than prior art in terms of dependence on mixing time. under which scenarios does this result reduce to \citep{bai2023regret} \cite{suttle2023beyond}? how are these results more/less general, due to assumptions on policy and critic function approximation error? where is hitting time dependence playing a role? also, we need to digest the answer to this question as well as the information contained in the remark after this theorem statement to create a table that we insert into page 2, to help illuminate the distinctiveness of our theorems.}

\begin{theorem}
\small
    \label{theorem_1_statement}
    Let $\{\theta_t\}_{t=1}^{T}$ be defined as in Lemma \ref{lem_framework}. If assumptions \ref{assumption:erogidcity}, \ref{assum:policy_conditions}, \ref{assump_transfer_error},  \ref{assump_4} hold,  $J(\cdot)$ is $L$-smooth, then the following inequality holds.
    \begin{align}
        \label{thm_final_convergence}
        \begin{split}
         %    &J^{*}-\frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\left[J(\theta_t)\right]\leq  \sqrt{\mathcal{E}^{actor}_{app}} + \\ &\wo{ \frac{G_H}{\sqrt{T}} \sqrt{\tau_{mix} \log T_{max}} } + \wo{ \frac{\sqrt{\tau_{mix} T_{\max}} \log T_{\max}}{T^{\frac{1}{8}}}} +\\ &\wo{
         % \frac{\sqrt{\tau_{mix}} (\log T_{\max})}{\sqrt{T}}} + \bo{\frac{\sqrt{\log(T_{max}) T_{max}} \mathcal{E}^{critic}_{app}}{\sqrt{T}}}  +\\ 
         %    &\wo{ \frac{\sqrt{\tau_{mix} \log T_{\max}}}{{T^{\frac{1}{4}}}}} 
         %    +\wo{ { \frac{\sqrt{\tau_{mix}\log T_{\max}}}{T_{\max}^{\frac{1}{2}}}}}  
        &J^{*}-\frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\left[J(\theta_t)\right]\leq  \sqrt{\mathcal{E}^{actor}_{app}}   + \wo{ \frac{\sqrt{\tau_{mix} T_{\max}} \log T_{\max}}{T^{\frac{1}{2}}}}  \\
         %    &\wo{
         % \frac{\sqrt{\tau_{mix}} (\log T_{\max})}{\sqrt{T}}} 
         % &+ \bo{\sqrt{\log(T_{max}) T_{max}} \mathcal{E}^{critic}_{app}}  
         &+\wo{ \frac{\sqrt{\tau_{mix} \log T_{\max}}}{{T^{\frac{1}{4}}}}} +\mathcal{E}^{critic}_{app}
            % &\wo{ \frac{\sqrt{\tau_{mix} \log T_{\max}}}{{T^{\frac{1}{4}}}}} 
        % +\wo{ { \frac{\sqrt{\tau_{mix}\log T_{\max}}}{\sqrt{T_{\max}}}}}.
        +\wo{  \sqrt{\frac{\tau_{mix}\log T_{\max}}{T_{\max}}}}.
        \end{split}
    \end{align}
\normalsize
\end{theorem}
% {\color{red} While now the analysis seems fine, the last term is not decaying. }
% Yes, agreed. Looking into it right now {\color{red} Thanks. }
The proof of this above theorem can be found in Appendix \ref{proof_of_thm1}. Here, we provide a proof sketch to highlight the main mechanics.
% \textcolor{red}{ALso make sure all the equations end with commas or periods. }

\textit{Proof sketch.} We rewrite the bound of the expectation of \ref{eq:general_bound} of Lemma \ref{lem_framework} into terms of \ref{eqn:31ss_2nd_moment} of Lemma \ref{lemma:31ss} and \ref{final_mac_bound} of Lemma \ref{lemma:convergence_rate}. 

The expectation of the second term of the RHS of \ref{eq:general_bound} can be bounded as the following using Lemma \ref{lemma:31ss} and Assumption \ref{assump_4},
\small

\begin{equation}\label{eq:exp_second_term}
    \begin{split}
         \frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\Vert h_t- h^*_t\Vert  \leq 
        \sqrt{\frac{1}{T}\sum_{t=1}^T \mathbf{E}\Vert h_t^{j_{max}} -\nabla J(\theta_t)\Vert^2} \\
        +\sqrt{\frac{2}{T}\sum_{t=1}^{T}\left(2+\dfrac{1}{\mu_F^2}\right)\mathbf{E}\bigg[\Vert \nabla_\theta J(\theta_t)\Vert^2\bigg]}.
        % \frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\Vert h_t- h^*_t\Vert  \leq 
        %  \sqrt{\frac{2}{T}\sum_{t=1}^{T}\mathbf{E}\bigg[\Vert  h_t\Vert^2\bigg]} \\
        % +\sqrt{\frac{2}{T}\sum_{t=1}^{T}\left(2+\dfrac{1}{\mu_F^2}\right)\mathbf{E}\bigg[\Vert \nabla_\theta J(\theta_t)\Vert^2\bigg]}.
    \end{split}
\end{equation}

\normalsize

For the third term of the RHS of \ref{eq:general_bound}, we can utilize Lemma \ref{lemma:42}
\small
\begin{equation}\label{eq:exp_third_term}
    \begin{split}
        \frac{R}{2T}\sum_{t=1}^{T}\alpha_t\Vert h_t\Vert^2  &\leq \frac{R}{T}\sqrt{\sum_{t=1}^{T}\Vert h_t\Vert^2}. 
        % = \frac{R}{\sqrt{T}\sqrt{T}}\sqrt{\sum_{t=1}^{T}\Vert h_t\Vert^2} \\ & \frac{R}{\sqrt{T}}\sqrt{\frac{1}{\sqrt{T}}\sum_{t=1}^{T}\Vert h_t\Vert^2}.
    \end{split}
\end{equation}

\normalsize
We can also bound the fourth term using the fact that it is a telescoping sum and that $\alpha_T < \alpha_t$, $\alpha_T = \frac{\alpha'_T}{\sum_{t=1}^{T}\Vert h_t\Vert^2}$,

\small
\begin{equation}
    \label{eq:second_bound_with_adagrad}
    \begin{split}
        \frac{1}{T}\sum_{t=1}^{T}&\frac{1}{\alpha_t}\mathbf{E}_{s\sim d^{\pi^*}}[\zeta_t]  \\&\leq \frac{\mathbf{E}_{s\sim d^{\pi^*}}[KL(\pi^*(\cdot\vert s)\Vert\pi_{\theta_1}(\cdot\vert s))]}{\alpha'_T}\frac{1}{T}\sqrt{\sum_{t=1}^{T}\Vert h_t\Vert^2}.
        % \\&=\frac{\mathbf{E}_{s\sim d^{\pi^*}}[KL(\pi^*(\cdot\vert s)\Vert\pi_{\theta_1}(\cdot\vert s))]\sqrt{\frac{1}{T}\sum_{t=1}^{T}\Vert h_t\Vert^2}}{\sqrt{T}\alpha'_T} .
    \end{split}
\end{equation}
\normalsize

\noindent We can now plug these bounds back into \ref{eq:general_bound} and ignore constants:. 
% Note when combining the $\sqrt{\frac{1}{T}\sum_{t=1}^{T}\Vert h_t\Vert^2}$ terms in \ref{eq:exp_second_term}, \ref{eq:exp_third_term}, and \ref{eq:second_bound_with_adagrad}, we get $\left(1 + \frac{2}{T}\right)\sqrt{\frac{1}{\sqrt{T}}\sum_{t=1}^{T}\Vert h_t\Vert^2} = \bo{1}\sqrt{\frac{1}{\sqrt{T}}\sum_{t=1}^{T}\Vert h_t\Vert^2} = \sqrt{\frac{1}{\sqrt{T}}\sum_{t=1}^{T}\Vert h_t\Vert^2}$ 


\small
\begin{equation}
    \label{eq:general_bound_expectation}
    \begin{split}
            J^{*}-&\frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\Vert J(\theta_t)\Vert
            \leq \sqrt{\mathcal{E}^{actor}_{app}} +\frac{1}{T}\sqrt{\sum_{t=1}^{T}\mathbf{E}\bigg[\Vert  h_t\Vert^2\bigg]}  \\& + \sqrt{\frac{1}{T}\sum_{t=1}^T \mathbf{E}\Vert h_t^{j_{max}} -\nabla J(\theta_t)\Vert^2} +\sqrt{\frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\bigg[\Vert \nabla_\theta J(\theta_t)\Vert^2\bigg]}. 
            % J^{*}-&\frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\Vert J(\theta_t)\Vert
            % \leq \sqrt{\mathcal{E}^{actor}_{app}}  \\&  +\sqrt{\frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\bigg[\Vert \nabla_\theta J(\theta_t)\Vert^2\bigg]} \\&+\sqrt{\frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\bigg[\Vert  h_t\Vert^2\bigg]} 
            % .
    \end{split}
\end{equation}
\normalsize

Bounding the the second and third term by the RHS with Lemmas \ref{lemma:31ss} and \ref{lemma:convergence_rate} respectively concludes the proof.

\textbf{Remark.} With Theorem \ref{theorem_1_statement}, we can recover the $\bo{T^{-\frac{1}{4}}}$ as in \cite{bai2023regret}. Furthermore, MAC has a tighter dependence on mixing time with $\wo{\sqrt{\tau_{mix}}}$ compared to the $\wo{\tau_{mix}^2}$ in \cite{bai2023regret} despite having no prior knowledge of mixing time due to the combination of MLMC gradient estimation and Adagrad stepsize. Similar to \cite{bai2023regret}, the independent $\mathcal{E}_{app}^{actor} \geq 0$ term accounts for the general policy parameterization. However, our bound has no dependence on hitting time like \cite{bai2023regret} as their dependence was a result of their advantage estimation algorithm described in Section \ref{section:ppgae}. 

% Our final theoretical result follows from setting the critic estimation error $\mathcal{E}(t)$ and critic approximation error $\mathcal{E}_{app}^{critic}$ both to $0$.

% \begin{corollary}\label{cor:critic_error_zero}
% With the same assumptions as Theorem \ref{theorem_1_statement} and by setting $\mathcal{E}(t) = \mathcal{E}_{app}^{critic} = 0$,
%     \begin{align}
%         \begin{split}
%          %    &J^{*}-\frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\left[J(\theta_t)\right]\leq  \sqrt{\mathcal{E}^{actor}_{app}} + \\ &\wo{ \frac{G_H}{\sqrt{T}} \sqrt{\tau_{mix} \log T_{max}} } + \wo{ \frac{\sqrt{\tau_{mix} T_{\max}} \log T_{\max}}{T^{\frac{1}{8}}}} +\\ &\wo{
%          % \frac{\sqrt{\tau_{mix}} (\log T_{\max})}{\sqrt{T}}} + \bo{\frac{\sqrt{\log(T_{max}) T_{max}} \mathcal{E}^{critic}_{app}}{\sqrt{T}}}  +\\ 
%          %    &\wo{ \frac{\sqrt{\tau_{mix} \log T_{\max}}}{{T^{\frac{1}{4}}}}} 
%          %    +\wo{ { \frac{\sqrt{\tau_{mix}\log T_{\max}}}{T_{\max}^{\frac{1}{2}}}}}  
%             J^{*}-\frac{1}{T}\sum_{t=1}^{T}\mathbf{E}&\Vert J(\theta_t)\Vert
%             \leq \sqrt{\mathcal{E}^{actor}_{app}}+
%             \wo{  \sqrt{ \frac{\tau_{mix}\log T_{\max}}{T_{\max}}}} \\ &+\wo{ \sqrt{\frac{\tau_{mix} \log T_{max}}{T}} }  + \bo{T^{-\frac{1}{4}} }.
%             %\wo{\sqrt{\frac{\tau_{mix}T_{max}}{T_{max}}}} + \wo{T^{-\frac{1}{4}}}.
%             %+ \wo{ \frac{\sqrt{\tau_{mix} T_{\max}} \log T_{\max}}{T^{\frac{1}{8}}}}  \\
%          %    &\wo{
%          % \frac{\sqrt{\tau_{mix}} (\log T_{\max})}{\sqrt{T}}} 
%         %  &+ \bo{\frac{\sqrt{\log(T_{max}) T_{max}} \mathcal{E}^{critic}_{app}}{\sqrt{T}}}  
%         %     % &\wo{ \frac{\sqrt{\tau_{mix} \log T_{\max}}}{{T^{\frac{1}{4}}}}} 
%         % +\wo{ { \frac{\sqrt{\tau_{mix}\log T_{\max}}}{\sqrt{T_{\max}}}}}  
%         \end{split}
%     \end{align}
% \end{corollary}
% The proof of Corollary \ref{cor:critic_error_zero} is a simplified version of the proof of Theorem \ref{theorem_1_statement} presented here where all terms that arise from the critic error in the supporting lemmas vanish.

% \textbf{Remark. } With Corollary \ref{cor:critic_error_zero}, we can recover the $\bo{T^{-\frac{1}{4}}}$ as in \cite{bai2023regret}. 

% \textcolor{red}{Vaneet: I dont see this - I see $T^{7/8}$ rather than $T^{3/4}$ - likely something wrong in above theorem statement}

% By choosing $T_{max} = \sqrt[4]{T}$ we get $\bo{T^{-\frac{1}{8}}}$ dependence. Although we do not recover the $\bo{T^{-\frac{1}{4}}}$ as in \cite{bai2023regret}, this $\bo{T^{-\frac{1}{8}}}$ dependence is due the critic and reward tracking error terms which were crucial in removing the need to know mixing time, allowing for a more practical policy gradient algorithm.

% \textcolor{red}{I'm concerned about the $\frac{1}{\sqrt{T_{\max}}}$ in the second to last term. I originally planning to set $T_{\max} = \sqrt[4]{T}$ and $\mathcal{E}^{critic}_{app} = 0$ to recover the $\bo{T^{-\frac{1}{4}}}$ but with this $\frac{1}{\sqrt{T_{\max}}}$ in the denominator of the second to last term we will instead get $\bo{T^{-\frac{1}{8}}}$}

% \textcolor{red}{I got a $\sqrt{\tau_{mix}}$ dependence but I not sure if I can recover the $\bo{T^{-\frac{1}{4}}}$ like in vaneet's paper. In fact, I'm concerned that this error grows with $T$ which doesn't make sense}

% \textcolor{red}{Another thing to note is that the $T$ is vaneet's paper is different from the $T$ in our paper. In his, $T$ is the total number of samples, and $K$ is the number of epochs/trajectories of length $H = 16 \tau_{mix}\tau_{hit}\sqrt{T}(\log T)^2$. In our ICML and in this latex file, $T$ is the number of trajectories of length of at most $T_{\max}$. I don't think that should fundamentally change anything...but not entirely sure.}
% \textcolor{red}{I guess maybe when we compare the dependence then it comes up. Because for them $T$ is total number of samples and for us it is $T*T_{\max}$ }

% ----------------------------------------

% Below is a different attempt to bound $\frac{1}{T}\sum_{t=1}^{T}\mathbf{E}\bigg[\Vert  h_t-\nabla_{\theta}J(\theta_t)\Vert^2\bigg]$ by breaking it using the definition of $h_t^{MLMC}$

% Let $h_t^N = \frac{1}{N}\sum^N_{i=1} h(\theta_t; s^i_t; a^i_t)$
% \begin{equation}
%     \label{gradient_error_bound_second_version}
%     \begin{split}
%     \frac{2}{T}\sum_{t=1}^{T}\mathbf{E}\bigg[\Vert  h_t-\nabla_{\theta}J(\theta_t)\Vert^2\bigg] =\frac{2}{T}\sum_{t=1}^{T}\sum_{t=1\mathbf{E}\bigg[\Vert  h^0_t+ 2^{J_t}(h^{2^{J_t}}_t - h^{2^{J_t-1}}_t )-\nabla_{\theta}J(\theta_t)\Vert^2\bigg] \leq \\ \frac{2}{T}\sum_{t=1}^{T}\mathbf{E}\bigg[\Vert  h^0_t+ T_{\max}(h^{T_{\max}}_t - h^{\frac{T_{\max}}{2}}_t )-\nabla_{\theta}J(\theta_t)\Vert^2\bigg] \leq \\ \frac{2}{T}\sum_{t=1}^{T}\mathbf{E}\bigg[\Vert  h^0_t \Vert^2 + \Vert T_{\max}h^{T_{\max}}_t -\nabla_{\theta}J(\theta_t)\Vert^2 + \Vert T_{\max}h^{\frac{T_{\max}}{2}}_t -\nabla_{\theta}J(\theta_t)\Vert^2\bigg] \leq \\ \frac{2}{T}\sum_{t=1}^{T}\bigg(\mathbf{E}\bigg[\Vert  h^0_t \Vert^2 \bigg] + \mathbf{E}\bigg[\Vert T_{\max}h^{T_{\max}}_t -\nabla_{\theta}J(\theta_t)\Vert^2\bigg] + \mathbf{E}\bigg[\Vert T_{\max}h^{\frac{T_{\max}}{2}}_t -\nabla_{\theta}J(\theta_t)\Vert^2\bigg]\bigg)
%     \end{split}
% \end{equation}

% The first term is $\mathbf{E}\bigg[\Vert  h^0_t \Vert^2 \bigg] \leq \bo{G_H^2}$

% In terms of growth rate, I think the second and third as the
